Incentivize without Bonus: Provably Efficient Model-based Online Multi-agent RL for Markov Games

Multi-agent reinforcement learning (MARL) lies at the heart of a plethora of applications involving the interaction of a group of agents in a shared unknown environment. A prominent framework for studying MARL is Markov games, with the goal of finding various notions of equilibria in a sample-efficient manner, such as the Nash equilibrium (NE) and the coarse correlated equilibrium (CCE). However, existing sample-efficient approaches either require tailored uncertainty estimation under function approximation, or careful coordination of the players. In this paper, we propose a novel model-based algorithm, called VMG, that incentivizes exploration via biasing the empirical estimate of the model parameters towards those with a higher collective best-response values of all the players when fixing the other players' policies, thus encouraging the policy to deviate from its current equilibrium for more exploration. VMG is oblivious to different forms of function approximation, and permits simultaneous and uncoupled policy updates of all players. Theoretically, we also establish that VMG achieves a near-optimal regret for finding both the NEs of two-player zero-sum Markov games and CCEs of multi-player general-sum Markov games under linear function approximation in an online environment, which nearly match their counterparts with sophisticated uncertainty quantification.

==> Value-incentivized-Game-arxiv/abstract.tex <==


\begin{abstract}

Multi-agent reinforcement learning (MARL) lies at the heart of a plethora of applications involving the interaction of a group of agents in a shared unknown environment. A prominent framework for studying MARL is Markov games, with the goal of finding various notions of equilibria in a sample-efficient manner, such as the Nash equilibrium (NE) and the coarse correlated equilibrium (CCE). 
However, existing sample-efficient approaches either require  tailored uncertainty estimation  under function approximation, or  careful coordination of the players. In this paper, we propose a novel model-based algorithm, called \name, that incentivizes exploration via biasing the empirical estimate of the model parameters towards those with a higher collective  best-response values of all the players when fixing the other players' policies, thus encouraging the policy to deviate from its current equilibrium  for more exploration. \name is oblivious to different forms of function approximation, and permits simultaneous and uncoupled policy updates of all players. Theoretically, we also establish that \name achieves a near-optimal regret for finding both the NEs of two-player zero-sum Markov games and  CCEs of multi-player general-sum Markov games under linear function approximation in an online  environment,  which nearly match their counterparts with sophisticated uncertainty quantification.  
 

\end{abstract}

==> Value-incentivized-Game-arxiv/defs.tex <==
\DeclareMathOperator*{\dom}{dom}
\DeclareMathOperator*{\Sp}{Sp} 
\DeclareMathOperator*{\sri}{sri}
\DeclareMathOperator*{\minimize}{minimize}
\DeclareMathOperator*{\loss}{loss}
\DeclareMathOperator*{\relint}{relint}
\DeclareMathOperator*{\Fix}{{Fix}}
\DeclareMathOperator*{\domain}{dom}
\DeclareMathOperator{\prox}{\mathbf{prox}}
\DeclareMathOperator{\thinprox}{prox}
\DeclareMathOperator{\Div}{Div}
\DeclareMathOperator{\Err}{Err}
\newcommand{\bigzero}{\mbox{\normalfont\Large\bfseries 0}}

\usepackage{xcolor}
\definecolor{mydarkblue}{rgb}{0,0.08,0.45}
\definecolor{mygreen}{rgb}{0.032, 0.6392, 0.2039}
\definecolor{mypurple}{HTML}{B266FF}

\newcommand{\cmark}{\textcolor{mygreen}{\ding{51}}}
\newcommand{\xmark}{\textcolor{red}{\ding{55}}}
\def\RR{{\mathbb R}}
\def\NN{{\mathbb N}}
\def\EE{{\mathbb E}}
\def\PP{{\mathbb P}}
\def\DD{{\boldsymbol{\Delta}}}
\def\xx{{\boldsymbol x}}
\def\XX{{\boldsymbol X}}
\def\ZZ{{\boldsymbol Z}}
\def\YY{{\boldsymbol Y}}
\def\uu{{\boldsymbol u}}
\def\UU{{\boldsymbol U}}
\def\rr{{\boldsymbol r}}
\def\ww{{\boldsymbol w}}
\def\yy{{\boldsymbol y}}
\def\vv{{\boldsymbol v}}
\def\ww{{\boldsymbol w}}
\def\zz{{\boldsymbol z}}
\def\KK{{\boldsymbol K}}
\def\CC{{\boldsymbol C}}
\def\TT{{\boldsymbol T}}
\def\LL{{\mathcal L}}
\def\X{{\mathcal X}}
\def\S{{\mathcal S}}
\def\A{{\mathcal A}}
\def\balpha{{\boldsymbol u}}
\def\defas{:=}
\newtheorem{conjecture}{Conjecture}
\newtheorem{axiom}{Axiom}
\newtheorem{fact}{Fact}

\def\RR{{\mathbb R}}
\def\CC{{\mathbb C}}
\def\NN{{\mathbb N}}
\def\EE{{\mathbb E}}
\def\DD{{\boldsymbol{\Delta}}}


\def\xx{{\boldsymbol x}}
\def\XX{{\boldsymbol X}}
\def\ZZ{{\boldsymbol Z}}
\def\YY{{\boldsymbol Y}}
\def\uu{{\boldsymbol u}}
\def\UU{{\boldsymbol U}}
\def\rr{{\boldsymbol r}}
\def\ww{{\boldsymbol w}}
\def\yy{{\boldsymbol y}}
\def\vv{{\boldsymbol v}}
\def\ww{{\boldsymbol w}}
\def\zz{{\boldsymbol z}}
\def\KK{{\boldsymbol K}}
\def\TT{{\boldsymbol T}}
\def\LL{{\mathcal L}}
\def\X{{\mathcal X}}
\def\balpha{{\boldsymbol u}}
\def\defas{:=}

\def\ge{{\geqslant}}
\def\le{{\leqslant}}


==> Value-incentivized-Game-arxiv/discussion.tex <==
 
\section{Conclusion}
\label{sec:conclusion}
In this paper, we introduced \name, a provably-efficient model-based algorithm for online MARL that balances  exploration and exploitation without requiring explicit uncertainty quantification. The key innovation lies in incentivizing the model estimation to maximize the best-response value functions across all players to implicitly drive exploration. In addition, \name is readily compatible with modern deep reinforcement learning architectures using function approximation, and is demonstrated to achieve a near-optimal regret under linear function approximation of the model class. We believe this work takes an important step toward making MARL more practical and scalable for real-world applications.

Several promising directions remain for future work. For example, designing a model-free counterpart of \name that can be used in conjunction with function approximation could be a valuable extension. Additionally, it will be interesting to develop the performance guarantee of \name under alternative assumptions of function approximation, such as general function approximation and independent function approximation across the players to tame the curse of dimensionality and multi-agency. Last but not least, it will be of interest to study the performance of \name under adversarial environments.
 


==> Value-incentivized-Game-arxiv/introduction.tex <==

\section{Introduction}

Multi-agent reinforcement learning (MARL) is emerging as a crucial paradigm for solving complex decision-making problems in various domains, including robotics, game theory, and machine learning~\citep{busoniu2008comprehensive}. While single-agent reinforcement learning (RL) has been extensively studied and theoretically analyzed, MARL is still in its infancy, and many fundamental questions remain unanswered. Due to the interplay of multiple agents in an unknown environment, one of the key challenges is the design of efficient strategies for exploration that can be seamlessly implemented in the presence of a large number of agents\footnote{In this paper, we use the term agent and player interchangeably.} without the need of complicated coordination among the agents. In addition, due to the large dimensionality of the state and action spaces, which grows exponentially with respect to the number of agents in MARL, it necessitate the adoption of function approximation to enable tractable planning in modern RL regimes.

A de facto approach in exploration in RL is the principle of optimism in the face of uncertainty \citep{lai1987adaptive}, which argues the importance of quantifying the uncertainty, known as the {\em bonus} term, in the pertinent objects, e.g., the value functions, and using their upper confidence bound (UCB) to guide action selection. This principle has been embraced in the MARL literature, leading a flurry of algorithmic developments \citep{liu2021sharp,bai2021sample,song2021can,jin2021v,li2022minimax,ni2022representation,cui2023breaking,wang2023breaking,dai2024refined} that claim provable efficiency in solving Markov games \citep{littman1994markov}, a standard model for MARL. However, a major downside of this approach is that constructing the uncertainty sets quickly becomes intractable as the complexity of function approximation increases, which often requiring a tailored approach. For example, near-optimal techniques for constructing the bonus function in the tabular setting cannot be applied for general function approximation using neural networks.

 
    
Therefore, it is of great interest to explore alternative exploration strategies without resorting to explicit uncertainty quantification, and can be adopted even for general function approximation. Our work is inspired by the pioneering work of \citet{kumar1982new}, which identified the need to regularize the maximum-likelihood estimator of the model parameters using its optimal value function to incentivize exploration, and has been successfully applied to bandits and  single-agent RL problems ~\citep{liu2020exploration,hung2021reward,mete2021reward,liu2024maximize} with matching performance of their UCB counterparts. However, this strategy of {\em value-incentivized} exploration has not yet been fully realized in the Markov game setting; a recent attempt \citep{liu2024maximize} addressed    two-player zero-sum Markov games, however, it requires  asymmetric updates and solving bilevel optimization problems with the lower level problem being a Markov game itself. 
These limitations motivate the development of more efficient algorithms for the general multi-agent setting while enabling symmetric and independent updates of the players. 
 We address the following question: 
\begin{center}
    \emph{Can we develop provably efficient algorithms for online multi-player general-sum Markov games with function approximation using value-incentivized exploration?}
\end{center} 


 

\subsection{Contribution}
 

In this paper, we propose a provably-efficient model-based framework, named \name (\emph{\textbf{V}alue-incentivized \textbf{M}arkov \textbf{G}ame solver}), for solving online multi-player general-sum Markov games with function approximation. 
\name  
incentivizes exploration via biasing the empirical estimate of the model parameters towards those with a higher collective {\em best-response} values of all the players when fixing the other players' policies, thus encouraging the policy to deviate from the equilibrium of the current model estimate for more exploration. This approach is oblivious to different forms of function approximation, bypassing the need of designing tailored bonus functions to quantity the uncertainty in standard approaches. \name also permits simultaneous and uncoupled policy updates of all players, making it more suitable when the number of players scales. Theoretically, we also establish that \name achieves a near-optimal regret for a number of game-theoretic settings under linear function approximation, which are on par to their counterparts requiring explicit uncertainty quantification. Specifically, our main results are as follows.
\begin{itemize} 
    \item For two-player zero-sum matrix games, \name  achieves a near-optimal regret on the order of $\widetilde{O}(d\sqrt{T})$,\footnote{The notation $\widetilde{O}(\cdot)$ hides logarithmic factors in the standard order-wise notation.} where $d$ is the dimension of the feature space and $T$ is the number of iterations for model updates.  This translates to a sample complexity of $\widetilde{O}(d^2/\varepsilon^2)$ for finding an $\varepsilon$-optimal NE in terms of the duality gap.
    \item For finite-horizon multi-player general-sum Markov games, under the linear mixture model of the transition kernel, \name achieves a near-optimal regret on the order of $\widetilde{\gO}(d\sqrt{H^3T})$, where $H$ is the horizon length, and $T$ is the number of iterations for model updates. This translates to a near-optimal  --- up to a factor of $H$ ---  complexity of $\widetilde{O}(Nd^2H^4/\varepsilon^2)$ samples or $\widetilde{O}(Nd^2H^3/\varepsilon^2)$ trajectories for finding an $\varepsilon$-optimal CCE in terms of the optimality gap, which is also applicable to  finding $\varepsilon$-optimal NE for two-player zero-sum Markov games. We also extend \name to the infinite-horizon setting, which achieves a sample complexity of $\widetilde{\gO}(Nd^2/ ((1-\gamma)^4\varepsilon^2 ))$ to achieve $\varepsilon$-optimality.
      
     
     \item The unified framework of \name allows its reduction to important special cases such as symmetric matrix games, linear bandits and single-agent RL, which not only recovers the existing reward-biased MLE framework  but also discovers new formulation that might be of independent interest. 

\end{itemize}

 
\subsection{Related work}
\label{sec:related}


We  discuss a few threads of related work, focusing on those with theoretical guarantees. 
 

\paragraph{Two-player matrix games.} Finding the equilibrium of two-player zero-sum matrix games has been studied extensively in the literature, e.g., \citet{mertikopoulos2018cycles,shapley1953stochastic,daskalakis2018last,wei2020linear}, where faster last-iterate linear convergence is achieved in the presence of KL regularization \citep{cen2021fast,zhan2023policy}. Many of the proposed algorithms focus on the tabular setting with full information, where the expected returns in each iteration can be computed exactly when the payoff matrix is given. More pertinent to our work, \citet{o2021matrix} considered matrix games with bandit feedback under the tabular setting, where only a noisy payoff from the players' actions is observed at each round, and proposed to estimate the payoff matrix using the upper confidence bounds (UCB) in an entry-wise manner~\citep{lai1987adaptive,bouneffouf2016finite}, as well as K-learning~\citep{o2021variational} that is akin to Thompson sampling \citep{russo2018tutorial}. Our work goes beyond the tabular setting, and proposes an alternative to UCB-based exploration that work seamlessly with different forms of function approximation.

 

\paragraph{Multi-player general-sum Markov games.} General-sum Markov games are an important class of multi-agent RL (MARL) problems \citep{littman1994markov}, and a line of recent works~\citep{liu2021sharp,bai2021sample,mao2023provably,song2021can,jin2021v,li2022minimax,sessa2022efficient} studied the non-asymptotic sample complexity for learning various equilibria in general-sum Markov games for the tabular setting under different data generation mechanisms. These works again rely heavily on carefully constructing confidence bounds of  the value estimates to guide data collection and obtain tight sample complexity bounds. In addition, policy optimization algorithms have also been developed assuming full information of the underlying Markov games, e.g., \citet{erez2023regret,zhang2022policy,cen2023faster}. 



\paragraph{MARL with linear function approximation.} Modern MARL problems often involve large state and action spaces, and thus require function approximation to generalize from limited data. Most theoretical results focus on linear function approximation, where the transition kernel, reward or value functions are assumed to be linear functions of some known feature maps. The linear mixture model of the transition kernel considered herein follows a line of existing works in both single-agent and multi-agent settings, e.g., \citet{ayoub2020model,chen2022almost,modi2020sample,jia2020model,chen2022almost,liu2024maximize}, which is subtly different from another popular linear model \citep{jin2020provably,wang2019optimism,yang2019sample,xie2020learning}, and these two models are not mutually exclusive in general~\citep{chen2022almost}. Moreover, \citet{ni2022representation,huang2022towards} considered general function approximation and \citet{cui2023breaking,wang2023breaking,dai2024refined} considered independent function approximation to allow more expressive function classes that lead to stronger statistical guarantees, which usually require solving complicated constrained optimization problems to construct the bonus functions. 

\paragraph{Uncertainty estimation in online RL.} Uncertainty estimation is crucial for efficient exploration in online RL. Common approaches are constructing the confidence set of the model parameters based on the observed data, which have been demonstrated to be provably near-optimal in the tabular and linear function approximation settings~\citep{jin2018q,agarwal2023vo} but have  limited success in the presence of function approximation in practice~\citep{gawlikowski2023survey}. Thompson sampling provides an alternative approach to exploration by maintaining a posterior distribution over model parameters and sampling from this distribution to make decisions, which however becomes generally intractable under complex function approximation schemes~\citep{russo2018tutorial}. Our approach draws inspiration from the reward-biased maximum likelihood estimation framework, originally proposed by \citet{kumar1982new}, which has been recently adopted in the context of bandits \citep{liu2020exploration,hung2021reward,cen2024value} and single-agent RL \citep{mete2021reward,liu2024maximize}. However, to the best of our knowledge, this work is the first to generalize this idea to the multi-player game-theoretic setting, which not only recovers but leads to new formulations for the single-agent setting.

  

\subsection{Paper organization and notation}

The rest of this paper is organized as follows. Section~\ref{sec:matrix_game} studies two-player zero-sum matrix games,  Section~\ref{sec:markov} focuses on episodic multi-player general-sum Markov games, and we conclude in Section~\ref{sec:conclusion}. The proofs as well as the extension to the infinite-horizon setting are deferred to the appendix.

\paragraph{Notation.}
We let $[n]$ denote the index set $\{1, \dots, n\}$. Let $I_n$ denote the $n\times n$ identity matrix, and inner product in Euclidean space \(\mathbb{R}^n\) by $\langle\cdot,\cdot\rangle$. We let $\Delta^n$ denote the $n$-dimensional simplex, i.e., $\Delta^n=\{x\in\mathbb{R}^n: x\geq 0,\sum_{i=1}^n x_i=1\}$. For any $x\in\mathbb{R}^n$, we let $\|x\|_p$ denote the $\ell_p$ norm of $x$, $\forall p\in[1,\infty]$. We let $\mathbb{B}^d_2(R)$ denote the $d$-dimensional $\ell_2$ ball of radius $R$. The Kullback-Leibler (KL) divergence between two distributions $P$ and $Q$ is denoted as $\KL{P}{Q}\coloneqq \sum_{x}P(x)\log\frac{P(x)}{Q(x)}$.  

==> Value-incentivized-Game-arxiv/markov_game.tex <==
 

\section{Multi-player General-sum Markov Games}\label{sec:markov}
 
We now turn to the more challenging setting of online multi-player general-sum Markov games, which includes the two-player zero-sum Markov game as a special case. 

\subsection{Problem setting}\label{sec:markov_setting}



\paragraph{Multi-player general-sum Markov game.} We consider an $N$-player general-sum episodic Markov game with a finite horizon denoted as $\gM_\PP\coloneqq(\gS,\gA,\PP, r, H)$, where $\gS$ is the state space, $\gA\coloneqq\gA_1\times\cdots\times\gA_N\coloneqq\prod_{n=1}^{N} \gA_n$ is the joint action space for all players, with $\gA_n$  the action space of player $n$, and
$H\in\NN_+$ is the horizon length. Let $\Delta(\gS)$ and $\Delta(\gA)$ denote the set of probability distributions over $\gS$ and $\gA$, respectively.  
$\PP=\{\PP_h\}_{h\in[H]}$ with $\PP_h:\gS\times\gA\rightarrow\Delta(\gS)$ is the inhomogeneous transition kernel: at step $h$, the probability of transitioning from state $s$ to state $s'$ by the action $\va=(a^1,\cdots,a^n)$ is $\PP_h(s'|s,\va)$. $r =\{r_h^n\}_{h\in[H],n\in[N]}$ stands for the reward function with
$r_h^n:\gS\times\gA\rightarrow[0,1]$ the reward of the $n$-th player at step $h$.

\paragraph{Markov policies.} In this paper, we focus on the class of Markov policies, where the policy of each player depends only on the current state, without dependence on the history. We let $\pi^n:\gS\times[H]\rightarrow \Delta(\gA)$ denote the policy of player $n$, and $\pi^n_h(\cdot|s)\in\Delta(\gA_n)$ denotes the probability distribution of the action of player $n$ at step $h$ given any state $s$. 
We let $\vpi=(\pi^1,\cdots,\pi^N):\gS\times[H]\rightarrow\Delta(\gA)$ denote the joint Markov policy (we assume all policies appear in this paper are Markovian, and we let \textit{joint policy} stands for joint Markov policy), where $\vpi_h(\cdot|s)\coloneqq (\pi_h^1,\cdots,\pi_h^N)(\cdot|s)\in\Delta(\gA)$ for all $s\in\gS$ and $h\in[H]$.  
 For any joint policy $\vpi$, we let $\vpi^{-n}$ denote the joint policy excluding player $n$. With a slight abuse of notation, we write $\vpi=(\pi^n,\vpi^{-n})$. In addition, a joint policy $\vpi$ is called a \textit{product policy} if $\pi^1,\cdots,\pi^N$ are executed independently, i.e., under policy $\vpi$, each player takes actions independently. We denote $\vpi = \pi^1\times \cdots \times \pi^N$ for a product policy.
 



 \paragraph{KL-regularized value function and Q-function.} 
 Given a joint policy $\vpi$, the KL-regularized state-value function (\textit{value function}) $V^{\vpi}_{h,n}: \gS\rightarrow\R$ and the KL-regularized state-action value function (\textit{Q-function}) $Q^{\vpi}_{h,n}:\gS\times\gA\rightarrow\R$ of the $n$-th player under $\vpi$ --- with regularization parameter $\beta\geq 0$ --- are respectively defined as
 \begin{subequations}
 \begin{align}
    \forall s\in\gS, h\in[H]:\quad V_{h,n}^{\vpi}(s) &\coloneqq \E_{\PP,\vpi}\left[\sum_{i=h}^H r_i^n(s_i,\va_i)-\beta\log\frac{\pi^n(a_i^n|s_i)}{\piref^n(a_i^n|s_i)}\bigg|s_h=s\right],\label{eq:V}\\
    \forall (s,\va)\in\gS\times\gA, h\in[H]:\quad Q_{h,n}^{\vpi}(s,\va) &\coloneqq r_h^n(s,\va) +  \E_{s'\sim\PP_h(\cdot|s,\va)}\left[V_{h+1,n}^{\vpi}(s')\right],\label{eq:Q}
 \end{align}
 \end{subequations}
 where $s_i$ and $\va_i$ are the state and action at step $i$, respectively, and $\allpiref:\gS\times[H]\rightarrow\Delta(\gA)$ is the reference policy. When the reference policy is a uniform distribution over the joint action space, the regularization becomes the entropy regularization. 
  In \eqref{eq:V}, $\pi^n(\cdot|s)$ (resp.~$\piref^n(\cdot|s)$) should be understood as the marginal distribution of player $n$ under joint distribution $\vpi(\cdot|s)$ (resp.~$\allpiref(\cdot|s)$),
 and we define $V_{H+1,n}^{\vpi}(s)=0$ for all $s\in\gS$ and $\beta\geq 0$. To simplify the notation, we define $V_n^{\vpi}\coloneqq V_{1,n}^{\vpi}$ and $Q_n^{\vpi}\coloneqq Q_{1,n}^{\vpi}$ for all $n\in[N]$.
We assume $\rho\in\Delta(\gS)$ is the initial state distribution, i.e., $s_1\sim\rho$. Furthermore, we define $V_n^\vpi(\rho)\coloneqq \E_{s\sim\rho}[V_n^\vpi(s)]$.
 

We let $\vpi=\pi^n\times\vpi^{-n}$ denote the policy profile where all players but the $n$-th player execute policy $\vpi^{-n}$, and the $n$-th player executes policy $\pi^n$ independent of the other players. For all $n\in[N]$, we define the best-response value function
\begin{align}\label{eq:V_dagger}
    \forall s\in\gS,h\in[H],n\in[N]:\quad V_{h,n}^{\star,\vpi^{-n}}(s)\coloneqq \max_{\pi^n:\gS\times[H]\rightarrow\Delta(\gA_n)} V_{h,n}^{\pi^n\times\vpi^{-n}}(s),
\end{align}
which is the optimal value of player $n$ when the policies of other agents are fixed by $\vpi^{-n}$.
Importantly, there exists at least one policy $\pi^{n,\star}(\vpi^{-n})$ that achieves the maximum in \eqref{eq:V_dagger} for all $s\in\gS$, and this policy is referred to the \textit{best-response policy} of player $n$ under joint policy $\vpi^{-n}$~\citep{shapley1953stochastic}.
 We also define 
 $$V_n^{\star,\vpi^{-n}}(\rho)\coloneqq \max_{\pi^n:\gS\times[H]\rightarrow\Delta(\gA_n)} V_n^{\pi^n\times\vpi^{-n}}(\rho).$$
One important thing to notice is that the best-response policy $\pi^{n,\star}(\vpi^{-n})$ does not depend on the initial state distribution $\rho$~\citep{mei2020global}.

\paragraph{Equilibria of Markov games.} In a multi-player general-sum Markov game, each agent aims to maximize its own value function, where the Nash equilibrium (NE)~\citep{nash1950non} and the coarse correlated equilibrium (CCE)~\citep{aumann1987correlated} are two widely studied solution concepts, whose definitions are as follows.
\begin{itemize}
    \item \textit{Nash equilibrium (NE):} a product policy $\vpi=\pi^1\times\cdots\times\pi^N$ is a Nash equilibrium of $\gM_\PP$ if
    \begin{align}\label{eq:def_NE}
            \forall s\in\gS, n\in[N]:\quad V_n^{\star,\vpi^{-n}}(s)=V_n^{\pi^n,\vpi^{-n}}(s).
    \end{align}
    \item \textit{Coarse correlated equilibrium (CCE):} a joint policy $\vpi$ is a CCE of $\gM_\PP$ if
    \begin{align}\label{eq:def_CCE}
            \forall s\in\gS, n\in[N]:\quad V_n^{\star,\vpi^{-n}}(s)\leq V_n^{\pi^n,\vpi^{-n}}(s).
    \end{align}
\end{itemize}
It is obvious that every NE is a CCE, but the converse is not true in general. In general, computing the NE in general-sum Markov games is intractable \citep{daskalakis2009complexity}, except for two-player zero-sum Markov games. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\paragraph{Goal: regret minimization.} 
To measure the proximity of a policy $\vpi$ to the equilibrium, we define the (average) sub-optimality gap of policy $\vpi$ w.r.t. the initial distribution $\rho$ as
\begin{align}\label{eq:gap}
    \gap{\vpi}\coloneqq \frac{1}{N}\sum_{n=1}^N \left(V_n^{\star,\vpi^{-n}}(\rho) - V_n^{\vpi}(\rho)\right).
\end{align}
A \textit{product} policy $\vpi$ is said to be an $\varepsilon$-approximate NE (abbreviated as $\varepsilon$-NE) if $\gap{\vpi}\leq \varepsilon$, and a \textit{joint} policy $\vpi$ is said to be an $\varepsilon$-approximate CCE (abbreviated as $\varepsilon$-CCE) if $\gap{\vpi}\leq \varepsilon$.
 

%
We aim to design a model-based framework that find the approximate NE or CCE of the Markov game $\gM_\PP$ in a provably efficient manner. Similar to the matrix game setting, we consider the following regret measure:
\begin{align}\label{eq:regret_MG}
 \regret(T)\coloneqq\sum_{t=1}^T\gap{\vpi_t}=\sum_{t=1}^T\frac{1}{N}\sum_{n=1}^N \left(V_n^{\star,\vpi_t^{-n}}(\rho) - V_n^{\vpi_t}(\rho)\right),
\end{align}
where $\vpi_t$ is the policy profile at time $t$. Our goal is to achieve a sublinear regret with respect to the number of rounds $T$, by carefully balancing the trade-off between exploration and exploitation, even under function approximation of the model class. 


\subsection{Algorithm development}\label{sec:markov_alg}

For simplicity, we will focus on the function approximation over the transition kernel of the Markov game assuming the reward function is fixed and deterministic, while it is straightforwardly to also incorporate the reward function approximation. We let $\gF$ denote the function class of the estimators of the transition kernel of the Markov game, and we denote the parameterized transition kernel as
$$\PP_f=(\PP_{f,1},\cdots,\PP_{f,H})\in\gF=\gF_1\times\cdots\gF_H,$$ 
where $\gF$ is the function class and $f$ is its parameterization.  We define the value function $V_{f,h,n}^{\vpi}$ under the transition kernel $\PP_f$ as
\begin{align}\label{eq:V_f}
    \forall s\in\gS, h\in[H]:\quad V_{f,h,n}^{\vpi}(s)\coloneqq \E_{\PP_f,\vpi}\left[\sum_{i=h}^H \left(r_i^n(s_i,\va_i)-\beta\log\frac{\pi^n(a_i^n|s_i)}{\piref^n(a_i^n|s_i)}\right)\bigg|s_h=s\right],
\end{align}
and the Q-function  $Q_{f,h,n}^{\vpi}$ is defined likewise.

Akin to the matrix game case, \name alternates between updating the model updates based on all the transitions observed so far, and collecting new trajectories using the updated policies.  Suppose that at the $t$-th iteration, the  current estimate of the transition kernel is $\PP_{f_{t-1}}$, and its corresponding NE or CCE is $\vpi_t$. \name alternates between the following two steps.
\begin{itemize}
\item {\em Value-incentivized model updates.} Given all the collected transitions $\gD_{t-1,h}$ at each step $h$ and the equilibrium policy $\vpi_t$, \name updates the model parameter $f_t$  via solving a regularized maximum likelihood estimation (MLE) problem as \eqref{eq:model_update_mg}, favoring models that {\em minimizes} the negative log-likelihood $\gL_t(f)$ of the model, i.e.
\begin{align}\label{eq:loss_mg}
    \gL_t(f)\coloneqq \sum_{h=1}^H\sum_{(s_h,\va_h,s_{h+1})\in\gD_{t-1,h}}-\log \PP_{f,h}(s_{h+1}|s_h,\va_h),
\end{align}
and {\em maximizes} the sum of the {\em best-response} values of each player when the other player's strategy is fixed at $\vpi_t^{-n}$. In words, the regularizer tries to encourage models that incentive the players to deviate from their current policy, resulting in better exploration. 

\item {\em Trajectory collection from best-response policy updates.} Using the updated model  $\PP_{f_{t}}$, \name updates the best-response policy $\widetilde{\pi}_t^n$ of each player while fixing the policy $\vpi_t^{-n}$ of the other player via \eqref{eq:policy_update_2_mg}. \name then collects new trajectories by following policy $\vpi_t$ and $(\widetilde{\pi}_t^n,\vpi_t^{-n})$ for all $n\in [N]$, and update the dataset. 
\end{itemize}
The complete procedure of \name is summarized in Algorithm~\ref{alg:markov_game}, where the function $\gamesolver(\gM_f)$ returns the NE or CCE of the Markov game $\gM_f$ by calling off-the-shelf solvers, e.g., \citet{cai2024near,zhang2022policy}. Note that we are primarily interested in finding the NE for two-player zero-sum Markov games, and the CCE for multi-player general-sum Markov games, due to computational tractability.


 
\paragraph{Comparison with MEX.} \citet[Algorithm~2]{liu2024maximize} proposed the MEX framework, which also considered using value functions as a means to incentive exploration for   two-player zero-sum Markov games. Their algorithm requires asymmetric updates --- and two sets of model parameters as a result --- of the max and min players, where the model update of the max player is regularized by the optimal value $V_f^{\star} = \max_{\pi^1}\min_{\pi^2} V_{1,1}^{\vpi}(\rho)$ of the Markov game, which is an expensive saddle-point optimization problem, and the model update of the min player is regularized by the best-response value function. In contrast, \name only leverages best-response value functions as a regularization, which is much easier to solve. \name also permits simultaneous  updates for all the players, making it amenable to multi-player general-sum Markov games. In contrast, MEX does not apply to this more general setting.

 


\begin{algorithm}[!thb]
    \caption{Value-incentivized Online Markov Game (\name)}
    \label{alg:markov_game}
    \begin{algorithmic}[1]
    \STATE \textbf{Input:} reference policies $\allpiref$, initial transition kernel estimate $f_0\in\gF$, regularization coefficient $\alpha>0$, iteration number $T$.
    \STATE \textbf{Initialization:} dataset $\gD_{0,h}\coloneqq \emptyset$, $\forall  h\in[H]$.  
    \FOR{$t = 1,\cdots,T$}
    \STATE $\vpi_t \leftarrow \gamesolver(\gM_{f_{t-1}})$. \trianglecomment{$\gamesolver(\gM_f)$ returns a CCE or NE of game $\gM_f$.}
    \STATE Model update: Update the estimator $f_t$ by minimizing the following objective:
    \begin{align}\label{eq:model_update_mg}         
        f_t=\argmin_{f\in\gF}\; \gL_t(f)  - \alpha \sum_{n=1}^N V_{f,n}^{\star,\vpi_t^{-n}}(\rho) .
    \end{align}
    \STATE Compute best-response policies $\{\widetilde{\pi}_t^n\}_{n\in[N]}$:
    \begin{align}\label{eq:policy_update_2_mg}
        \forall n\in[N]:\quad \widetilde{\pi}_t^n& = \argmax_{\pi^n:\gS\times[H]\rightarrow\Delta(\gA_n)} V_{f_t,n}^{\pi^n,\vpi_t^{-n}}(\rho).
    \end{align}
    \STATE Data collection: 
    sample a trajectory with transition tuples $\{(s_{t,h},\va_{t,h}, s_{t,h+1})\}_{h=1}^H$ by executing $\vpi_t$, and sample a trajectory with transition tuples $\{(s_{t,h}^n,\va_{t,h}^n, s_{t,h+1}^n)\}_{h=1}^H$ by executing $(\widetilde{\pi}_t^n,\vpi_t^{-n})$
    for each $n\in[N]$.
    Update the dataset  $\gD_{t,h} = \gD_{t-1,h}  \cup_{n=1}^N \{ (s_{t,h},\va_{t,h},s_{t,h+1}), (s_{t,h}^n,\va_{t,h}^n,s_{t,h+1}^n) \}$, $\forall h\in[H]$.  
    \ENDFOR 
    \end{algorithmic}
\end{algorithm}
 

\paragraph{Reduction to the single-agent MDP case.} \name can be reduced to the Markov decision process (MDP) setting via either setting the number of players $N=1$  in the multi-player general-sum Markov game, or setting the action space of the min player  to a singleton in the two-player zero-sum Markov game. Interestingly, the former leads to the value regularization $V_{f}^{\star}(\rho)$ studied in MEX \citep{liu2024maximize}, while the latter leads to a new form of regularizer $V_{f}^{\star}(\rho)-V_{f}^{\pi_t}(\rho)$, adding friction from the current policy $\pi_t$. 

 
 

\subsection{Theoretical guarantee}\label{sec:markov_analysis}

We demonstrate that \name achieves near-optimal regret under the following linear mixture model of the transition kernel for Markov games.


\begin{asmp}[linear mixture model]\label{asmp:function_class}
    The function class $\gF=\gF_1\times\cdots\gF_H$ is
    $$\forall h\in[H]:\quad\gF_h\coloneqq\left\{f_h|f_h(s'|s,\va)=\phi_h(s,\va,s')^\top{\theta_h},\quad \forall (s,\va,s')\in\gS\times\gA\times\gS,\theta_h\in\Theta_h\right\},$$
    where $\phi_h=(\phi_h^1,\cdots,\phi_h^d):\gS\times\gA\times\gS\rightarrow\R^d$ are the known feature maps with $\phi_h^i:\gS\times\gA\rightarrow\Delta(\gS)$ being transition kernels for all $i\in[d]$. $\norm{\phi_h(s,\va,s')}_2\leq 1$ for all $(s,\va,s')$, and $\Theta_h\subseteq\mathbb{B}^d_2(\sqrt{d})$, $\forall h\in[H]$. For each $f_h\in\gF_h$ and $(s,\va)\in\gS\times\gA$, $f_h(\cdot|s,\va)\in\Delta(\gS)$, $\forall h\in[H]$.
\end{asmp}
The linear mixture model is a common assumption in the RL literature, see, for example, \citet{ayoub2020model,modi2020sample,cai2020provably} for  single-agent RL, and \citet{chen2022almost,liu2024maximize} for Markov games.
We also assume the function class $\gF$ is expressive enough to describe the true transition kernel of the Markov game.
\begin{asmp}[realizability]\label{asmp:realizable}
    There exists $f^\star\in\gF$ such that $\PP_{f^\star}=\PP$.
\end{asmp}

\paragraph{Regret guarantee.} We now present our main result for the regret of the online Markov game, whose  proof is deferred to Appendix~\ref{app:proof_thm_regret_MP}. 
\begin{thm}\label{thm:regret_MG}
    Under Assumptions~\ref{asmp:function_class} and \ref{asmp:realizable}, if setting the regularization coefficient $\alpha$ as
    $$\alpha = \sqrt{\frac{ T}{Hd\log\left(1+\frac{T^{3/2}H^2}{\sqrt{d}}\right)} \left( \log\left(\frac{HN}{\delta}\right) + d\log\left(d|\gS|T\right) \right) },$$
    then for any $\beta\geq 0$, with any initial state distribution $\rho$, transition kernel estimator $f_0\in\gF$ and reference policy $\allpiref$, the regret of Algorithm~\ref{alg:markov_game} satisfies the following bound with probability at least $1-\delta$ for any $\delta\in(0,1)$:
    \begin{align}\label{eq:regret_MG_bd}
        \forall T\in\NN_+:\quad\regret(T)\leq \widetilde{\gO}\left(d \sqrt{H^3T}\cdot\sqrt{\frac{1}{d}\log\left(\frac{NH}{\delta}\right) + \log\left(d|\gS|T\right) 
        }\right).
    \end{align}
\end{thm}
Theorem~\ref{thm:regret_MG} establishes that by setting $\alpha$ on the order of $\widetilde{O}(\sqrt{T/H})$, with high probability, the regret of \name is no larger than an order of
$$ \widetilde{\gO}\left(d \sqrt{H^3T}\right)$$
for general-sum Markov games. When reducing to  two-player zero-sum Markov games, our  regret bound --- established for both players --- matches that of MEX~\citep{liu2024maximize}, which only covers  the max player. To the best of our knowledge, this is the first result that establishes a near-optimal sublinear regret for general-sum Markov games without explicit uncertainty quantification via constructing bonus functions or uncertainty sets. 

In addition, since
$    \min_{t\in[T]}\gap{\vpi_t}\leq  \regret(T) / T$ and each iteration collects $N+1$ trajectories, \name is guaranteed to find an $ \varepsilon$-NE ($\varepsilon$-CCE) of $\gM_\PP$ for any $\varepsilon>0$ within
$\widetilde{\gO}\left(\frac{ Nd^2H^3}{\varepsilon^2}\right)$ trajectories
or
$\widetilde{\gO}\left(\frac{ N d^2 H^4}{\varepsilon^2}\right)$ samples. Compared to the minimax sample complexity \citep{chen2022almost}, our sample complexity is near-optimal up to a factor of $H$ when the number of players $N$ is fixed.

  

%\begin{crl}[iteration/sample complexity of the Markov game]\label{crl:complexity_MG}
%    Under the same setting as in Theorem~\ref{thm:regret_MG}, for any $\beta\geq 0$, with any initial state distribution $\rho$, transition kernel estimator $f_0\in\gF$ and reference policy $\allpiref$, if $\gamesolver(\gM_{f_t})$ returns the NE (CCE) of the Markov game $\gM_{f_t}$ in each iteration $t$ of Algorithm~\ref{alg:markov_game}, then with probability at least 1-$\delta$,
%Algorithm~\ref{alg:markov_game} finds an $\varepsilon$-NE ($\varepsilon$-CCE) of $\gM_\PP$ for any $\varepsilon>0$ within
%$T=\widetilde{\gO}\left(\frac{H^3 d^2}{\varepsilon^2}\right)$
%iterations and with a sample complexity 
%$\widetilde{\gO}\left(\frac{H^4 N d^2}{\varepsilon^2}\right)$.
%\end{crl}



 

 
     

==> Value-incentivized-Game-arxiv/math_commands.tex <==
\usepackage{amsmath,amsfonts,bm}
\usepackage{algorithm,algorithmic}

% Mark sections of captions for referring to divisions of figures
%\newcommand{\figleft}{{\em (Left)}}
%\newcommand{\figcenter}{{\em (Center)}}
%\newcommand{\figright}{{\em (Right)}}
%\newcommand{\figtop}{{\em (Top)}}
%\newcommand{\figbottom}{{\em (Bottom)}}
%\newcommand{\captiona}{{\em (a)}}
%\newcommand{\captionb}{{\em (b)}}
%\newcommand{\captionc}{{\em (c)}}
%\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
%\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
%\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
%\newcommand{\train}{\mathcal{D}}
%\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
%\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vxi{{\bm{\xi}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\vphi{{\bm{\varphi}}}
\def\vpi{{\bm{\pi}}}
\def\vpsi{{\bm{\zeta}}}
\def\vomega{{\bm{\omega}}}
\def\vdelta{{\bm{\delta}}}
\def\valpha{{\bm{\alpha}}}
\def\vzeta{{\bm{\zeta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}
\def\vtheta{{\bm{\theta}}}
\def\vnu{{\bm{\nu}}}
\def\vlmd{{\bm{\lambda}}}
\def\vbeta{{\bm{\beta}}}

\def\tf{{\tilde f}}

% Matrices
\def\mI{{\bm{I}}}
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mM{{\bm{M}}}

% time derivatives of f-ns
\def\dX{{\dot{X}}}
\def\dY{{\dot{Y}}}
\def\dZ{{\dot{Z}}}
\def\ddX{{\ddot{X}}}
\def\ddY{{\ddot{Y}}}
\def\ddZ{{\ddot{Z}}}

% time derivatives of v-rs
\def\dvx{{\dot{\vx}}}
\def\dvy{{\dot{\vy}}}
\def\dvz{{\dot{\vz}}}
\def\dvw{{\dot{\vw}}}
\def\dvom{{\dot{\vomega}}}
\def\ddvx{{\ddot{\vx}}}
\def\ddvy{{\ddot{\vy}}}
\def\ddvz{{\ddot{\vz}}}
\def\ddvw{{\ddot{\vw}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
%\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
%\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
%\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
%\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
%\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
%\newcommand{\pmodel}{p_{\rm{model}}}
%\newcommand{\Pmodel}{P_{\rm{model}}}
%\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
%\newcommand{\pencode}{p_{\rm{encoder}}}
%\newcommand{\pdecode}{p_{\rm{decoder}}}
%\newcommand{\precons}{p_{\rm{reconstruct}}}

%\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
%\newcommand{\KL}[2]{\textnormal{KL}\left(#1\|#2\right)}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

%\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.
%
% \DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\argmin}{arg\,min}
% \DeclareMathOperator*{\argmax}{argmax}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\geom}{Geom}
\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\diag}{diag}

%\DeclareMathOperator{\sign}{sign}
%\DeclareMathOperator{\Tr}{Tr}
%\let\ab\allowbreak
\usepackage{amssymb}
% \usepackage{ wasysym } 

==> Value-incentivized-Game-arxiv/matrix_game.tex <==

\section{Two-Player Zero-Sum Matrix Games}
\label{sec:matrix_game}

In this section, we start with a simple setting of two-player zero-sum matrix games, to develop our algorithmic framework.

\subsection{Problem setting}\label{sec:matrix_setting}


\paragraph{Two-player zero-sum matrix game.} 
We consider the (possibly KL-regularized) two-player zero-sum matrix games with the following objective:
\begin{align}\label{eq:game_obj}
    \max_{\mu\in\Delta^m} \min_{\nu\in\Delta^{n}} \; f^{\mu,\nu}(A)\coloneqq\mu^\top A \nu - \beta\KL{\mu}{\muref} + \beta\KL{\nu}{\nuref},
\end{align}
where $A\in\mathbb{R}^{m\times n}$ is the payoff matrix, $\mu\in\Delta^m$ and $\muref\in\Delta^m$ (resp. $\nu\in\Delta^n$ and $\nuref\in\Delta^n$) are the policy and reference policy for the max (resp. min) player, and $\beta\geq 0$ is the regularization parameter.\footnote{For simplicity, we set the same regularization parameter for both players; our analysis continues to hold with different regularization parameters $\beta_1$ and $\beta_2$ for each player.} Here, the reference policies can be used to incorporate prior knowledge or preference of the game; when the reference policies are uniform distributions, the KL regularization becomes entropy regularization, which are studied in, e.g., \citet{cen2021fast}.

 
\paragraph{Nash equilibrium.} The policy pair $(\mu^\star,\nu^\star)$ corresponding to the solution to the saddle-point problem \eqref{eq:game_obj} represents a desirable state of the game, where both players perform their (regularized) best-response strategies against  the other player, so that no players will unitarily deviate from its current policy. Specifically,  the policy pair $(\mu^\star,\nu^\star)$ satisfies
$$\forall (\mu,\nu)\in\Delta^m\times\Delta^n:\quad f^{\mu,\nu^\star}(A)\leq f^{\mu^\star,\nu^\star}(A)\leq f^{\mu^\star,\nu}(A), $$
and is called the {\em Nash equilibrium} (NE) of the matrix game \citep{nash1950non}.\footnote{We note that under entropy regularization, the equilibrium is also known as the {\em quantal response equilibrium} (QRE) \citep{mckelvey1995quantal} when $\beta>0$.}

\paragraph{Noisy bandit feedback.}
We are interested in learning the NE when the payoff matrix $A$ is unknown and can only be accessed through a stochastic oracle. Specifically, for any $i\in[m]$ and $j\in[n]$, 
we can query the entry $A(i,j)$, and receive a noisy feedback $\widehat{A}(i,j)$ of $A(i,j)$ from an oracle, i.e.,
\begin{align}\label{eq:noisy_feedback}
    \widehat{A}(i,j) = A(i,j) + \xi,
\end{align}
where the noise $\xi$ is an i.i.d. zero-mean random variable across different queries. Each of the collected data tuple is thus in the form of $(i,j, \widehat{A}(i,j) )$.
 

\paragraph{Goal: regret minimization.} Our goal is to design an easy-to-implement framework that can find the approximate NE of the matrix game \eqref{eq:game_obj} with as few queries as possible to the stochastic oracle in a sequential manner. To begin, we define the following 
\begin{align}\label{eq:f_notation}
    f^{\star,\nu}(A)\coloneqq \max_{\mu\in\Delta^m} f^{\mu,\nu}(A),\quad f^{\mu,\star}(A)\coloneqq \min_{\nu\in\Delta^n} f^{\mu,\nu}(A),\quad\text{and}\quad f^\star(A)\coloneqq \max_{\mu\in\Delta^m}\min_{\nu\in\Delta^n} f^{\mu,\nu}(A)
\end{align}
for any payoff matrix $A$. The duality gap of the matrix game \eqref{eq:game_obj} at a policy pair $(\mu,\nu)$ is defined as
\begin{align}\label{eq:dualgap}
    \dualgap{\mu,\nu}\coloneqq    f^{\star,\nu}(A) - f^{\mu,\star}(A) ,
\end{align}
where it is evident that $ \dualgap{\mu^{\star},\nu^{\star}} = 0$. A policy pair $(\mu,\nu)$ is called an $\varepsilon$-approximate NE (abbreviated as $\epsilon$-NE) of the matrix game \eqref{eq:game_obj} if $\dualgap{\mu,\nu}\leq \varepsilon$.

In an online setting, given a sequence of policy updates $\{(\mu_t, \nu_t)\}_{t=1,\ldots, T}$ over $T$ rounds, a common performance metric is the cumulative regret, defined as 
\begin{align}\label{eq:regret}
    \regret(T)&\coloneqq \sum_{t=1}^T\dualgap{\mu_t,\nu_t}  = \underbrace{ \sum_{t=1}^T \left(  f^{\star,\nu_t}(A)-f^\star(A) \right) }_{\text{regret for min-player}}  + \underbrace{  \sum_{t=1}^T \left( f^\star(A) - f^{\mu_t,\star}(A) \right) }_{\text{regret for max-player}},
\end{align}
which encapsulates the regret from both players. Our goal is to achieve a sublinear, and ideally near-optimal, regret with respect to the number of rounds $T$, by carefully balancing the trade-off between exploration and exploitation, even under function approximation of the model class. 
 

\subsection{Algorithm development}\label{sec:matrix_alg}

We propose a model-based approach, called \name, that enables provably efficient exploration-exploitation trade-off via resorting to a carefully-regularized model (i.e., the payoff matrix) estimator without constructing uncertainty intervals. To enable function approximation, we parameterize the payoff matrix by $A_{\omega} \in \mathbb{R}^{m\times n}$,  where $\omega\in\Omega\subset\mathbb{R}^d$ is some vector in the parameter space $\Omega$. 

The proposed approach, on a high level, alternates between updating the payoff matrix based on all the samples collected so far, and collecting new samples using the updated  policies. Let's elaborate a bit further. At each round $t$, let  the current payoff matrix estimate be $A_{\omega_{t-1}}$, and its corresponding NE be $(\mu_t, \nu_t)$. 
\begin{itemize}
\item {\em Value-incentivized model updates.} Given all the collected data tuples $\gD_{t-1}$ and the policy pair $(\mu_t, \nu_t)$, \name updates the model parameter $\omega_t$  via solving a regularized least-squares estimation problem as \eqref{eq:model_update}, favoring models that {\em minimizes} the squared loss between the model and the noisy feedback stored in $\gD_{t-1}$, and {\em maximizes} the value of each player when the other player's strategy is fixed. In other words, the regularization term aims to maximize the duality gap at $(\mu_t, \nu_t)$, which tries to pull the model away from its current estimate $A_{t-1}$, whose duality gap is $0$ at $(\mu_t, \nu_t)$. The regularized estimator thus strikes a balance of exploitation (via least-squares on $\gD_{t-1}$) and exploration (via regularization against the current model $A_{\omega_{t-1}}$).

\item {\em Data collection from best-response policy updates.} Using the updated payoff matrix $A_{\omega_t}$, \name updates the best-response policy of each player while fixing the policy of the other player via \eqref{eq:policy_update_2}, resulting in policy pairs $(\widetilde{\mu}_t,\nu_t)$ and $(\mu_t,\widetilde{\nu}_t)$. Finally, \name collects one new sample from each of the policy pairs respectively following the oracle \eqref{eq:noisy_feedback}, and add them to the dataset $\gD_{t-1}$ to form $\gD_t$. 

\end{itemize}
The complete procedure of \name is summarized in Algorithm~\ref{alg:matrix_game}. \name invokes the mechanism of regularization as a means for incentivizing exploration, rendering it more amenable to implement in the presence of function approximation. In contrast, prior approach \citep{o2021matrix} heavily relies on 
explicitly adding an exploration bonus to the estimate of the payoff matrix using confidence intervals, which is challenging to construct under general function approximation. In addition, \name allows parallel and independent policy execution from both players.


 
\begin{algorithm}[th]
    \caption{Value-incentivized Online Matrix Game (\name)}
    \label{alg:matrix_game}
    \begin{algorithmic}[1]
    \STATE \textbf{Input:}  initial parameter $\omega_0$, regularization coefficient $\alpha>0$, iteration number $T$.  
    \STATE \textbf{Initialization:} dataset $\gD_0\coloneqq \emptyset$.
    \FOR{$t = 1,\cdots,T$}
    \STATE 
    Compute the Nash equilibrium $(\mu_t,\nu_t)$ of  the matrix game with the current parameter $\omega_{t-1}$:
    \begin{align}\label{eq:policy_update}
        \mu_t&=\argmax_{\mu\in\Delta^m}\min_{\nu\in\Delta^n}\; f^{\mu,\nu}(A_{\omega_{t-1}}),\qquad \nu_t=\argmin_{\nu\in\Delta^n}\max_{\mu\in\Delta^m}\; f^{\mu,\nu}(A_{\omega_{t-1}}).
    \end{align} 
    \STATE Model update: Update the parameter $\omega_t$ by minimizing the following objective:
    \begin{align}\label{eq:model_update}
        \omega_t=\argmin_{\omega\in\Omega}\sum_{(i,j,\widehat{A}(i,j))\in\gD_{t-1}}\left(A_\omega(i,j)-\widehat{A}(i,j)\right)^2  \underbrace{ -\alpha f^{\star, \nu_t}(A_{\omega})+\alpha f^{\mu_t,\star}(A_{\omega})}_{\textrm{value-incentivized~reg.}}.
    \end{align}
    \STATE Compute $\widetilde{\mu}_t$ and $\widetilde{\nu}_t$ by solving the following optimization problems:
    \begin{align}\label{eq:policy_update_2}
        \widetilde{\mu}_t& = \argmax_{\mu\in\Delta^m}\; f^{\mu,\nu_t}(A_{\omega_t}),\qquad \widetilde{\nu}_t = \argmin_{\nu\in\Delta^n}\; f^{\mu_t,\nu}(A_{\omega_t}).
    \end{align}
    \STATE Data collection: Sample $(i_t,j_t)\sim (\widetilde{\mu}_t,\nu_t)$ and $(i'_t,j'_t)\sim (\mu_t,\widetilde{\nu}_t)$ and get the noisy feedback $\widehat{A}(i_t,j_t)$ and $\widehat{A}(i'_t,j'_t)$ following the oracle \eqref{eq:noisy_feedback}. Update the dataset ${\gD}_t=\gD_{t-1}\cup\left\{ (i_t,j_t,\widehat{A}(i_t,j_t) ), \, (i'_t,j'_t,\widehat{A}(i'_t,j'_t) )\right\}$.
    \ENDFOR 
    \end{algorithmic}
\end{algorithm}

\paragraph{The benefit of regularization.} While \name is agnostic to the power of KL regularization in \eqref{eq:game_obj}, the major benefit of regularization comes in terms of computational efficiency. When the KL regularization parameter $\beta>0$, common first-order game solvers such as mirror descent ascent~\citep{sokota2022unified} or policy extragradient~\citep{cen2021fast} achieve a last-iterate  linear convergence rate when solving the matrix game \eqref{eq:policy_update}. Turning to the model update, when $\beta>0$, the regularization term in \eqref{eq:model_update} can be computed in closed form:
\begin{align}\label{eq:regularization_closed_form}
    & -  f^{\star,\nu_t}(A_\omega)+   f^{\mu_t,\star}(A_\omega) \notag\\
    &= - \beta\left[\log\left(\sum_{i=1}^n \mu_{\mathsf{ref},i} \exp\left(\frac{A_{\omega}(i,:)\nu_t}{\beta}\right)\right) +\log\left(\sum_{j=1}^m \nu_{\mathsf{ref},j} \exp\left(-\frac{\mu_t^\top A_{\omega}(:,j)}{\beta}\right)\right)\right]+C,
\end{align}
where $\mu_{\mathsf{ref},i}$ (resp. $\nu_{\mathsf{ref},j}$) is the $i$-th (resp. $j$-th) entry of $\mu_{\mathsf{ref}}$ (resp. $\nu_{\mathsf{ref}}$), $A_{\omega}(i,:)$ (resp. $A_{\omega}(:,j)$) is the $i$-th row (resp. $j$-th column) of $A_{\omega}$, and $C$ is a constant that does not depend on $A_\omega$. Leveraging the closed-form expression, one can bypass solving a bi-level optimization problem \eqref{eq:model_update} on its surface, but resorts to more efficient first-order methods. Last but not least, the policies $\widetilde{\mu}_t$ and $\widetilde{\nu}_t$ in \eqref{eq:policy_update_2} can be computed in closed form as well:
\begin{align}\label{eq:tilde_pi_closed_form}
    \widetilde{\mu}_{t,i} \propto \mu_{\mathsf{ref},i} \exp\left(\frac{A_{\omega_t}(i,:)\nu_t}{\beta}\right) ,\qquad \widetilde{\nu}_{t,j} \propto  \nu_{\mathsf{ref},j} \exp\left(-\frac{\mu_t^\top A_{\omega_t}(:,j)}{\beta}\right) ,\quad \forall i\in[m], j\in[n].
\end{align}


\paragraph{The case of symmetric payoff.} One important special class of matrix games is the symmetric matrix game~\citep{cheng2004notes}, with $A=-A^\top$, $\muref=\nuref$, and $m=n$. Many well-known games are symmetric, from classic games like rock-paper-scissors to the recent example of LLM alignment~\citep{munos2023nash,swamy2024minimaximalist,yang2024faster}. For a symmetric matrix game, it admits a symmetric Nash $(\mu^\star,\mu^\star)$, and Algorithm~\ref{alg:matrix_game}  reduces to a single-player algorithm by only tracking a single policy $\mu_t$, recognizing $\mu_t=\nu_t$ and $\widetilde{\mu}_t= \widetilde{\nu}_t$ due to $f^{\mu,\nu}(A)=-f^{\nu,\mu}(A)$. In addition,  \name only needs to collect one sample from the policy pair $(\widetilde{\mu}_t,\mu_t)$ in each iteration. This is particularly desirable when the policy is expensive to store and update, such as large-scale neural networks or LLMs. 

\paragraph{Reduction to the bandit case.} By setting the action space of the min player to $n=1$, \name seamlessly reduces to the bandit setting, where the payoff matrix becomes a reward vector $A \in \mathbb{R}^m$. Here, we let $f^{\mu}(A) = \mu^{\top} A - \beta\KL{\mu}{\muref}$ and 
     $f^{\star}(A)\coloneqq \max_{\mu\in\Delta^m} f^{\mu}(A)$. Interestingly, to encourage exploration, the regularization term favors a reward estimate that maximizes its regret $  f^{\star}(A_{\omega}) -  f^{\mu_t}(A_{\omega})$ on the current policy $\mu_t$, which is {\em different from} the reward-biasing framework that only regularizes against $  f^{\star}(A_{\omega})$ \citep{cen2024value,liu2020exploration}.   

\subsection{Theoretical guarantee}\label{sec:matrix_analysis}

We demonstrate that \name achieves near-optimal regret, assuming linear function approximation of the payoff matrix. Specifically, we have the following assumption.

\begin{asmp}[Linear function approximation]\label{asmp:bounded_payoff}
The payoff matrix is parameterized as  
\begin{align}\label{eq:A_param}
    A_\omega(i,j)\coloneqq \phi(i,j)^\top \omega, \quad\forall i\in[m], j\in[n],
\end{align}
where $\omega\in\Omega\subset\mathbb{R}^d$ is the parameter vector and $\phi(i,j)\in\mathbb{R}^d$ is the feature vector for the $(i,j)$-th entry. Here, the feature vectors are known and fixed, and satisfy $\norm{\phi(i,j)}_2\leq 1$ for all $i\in[m]$ and $j\in[n]$. For all $ \omega\in\Omega$, we suppose $\norm{\omega}_2\leq \sqrt{d}$ and $\norm{A_\omega}_{\infty}\leq B_l$ for some $B_l>0$. 
\end{asmp}

 

We also assume that the linear function class is expressive enough to describe the true payoff matrix $A$.
\begin{asmp}[realizability]\label{asmp:expressive}
    There exists $\omega^\star\in\Omega$ such that $A_{\omega^\star}=A$.
\end{asmp}

Next, we impose the noise follows standard sub-Gaussian distribution.
\begin{asmp}[i.i.d. sub-Gaussian noise]\label{asmp:noise}
    The noise $\xi$ in \eqref{eq:noisy_feedback} are i.i.d. mean-zero sub-Gaussian random variables with sub-Gaussian parameter $\sigma>0$.
\end{asmp}

\paragraph{Regret guarantee.} The following theorem states the regret bound of \name under appropriate choice of the regularization parameter.  
\begin{thm}\label{thm:regret}
    Suppose Assumptions~\ref{asmp:bounded_payoff}, \ref{asmp:expressive} and \ref{asmp:noise} hold. Let $\delta\in(0,1)$, setting the 
regularization coefficient $\alpha$ as
\begin{align}\label{eq:alpha}
\alpha=\sqrt{\frac{T}{d\log\left(1+(T/d)^{3/2}\right)} \left(\log(4T/\delta)+d\log (dT)\right)},
\end{align}
then for any $\beta\geq 0$, with any initial parameter $\omega_0$ and reference policies $\muref$ and $\nuref$, we have with probability at least $1-\delta$,
    \begin{align}\label{eq:regret_bound}
  \regret(T)=\gO\left(B_l\left(B_l+\sigma\sqrt{2\log(8T/\delta)}\right)d\sqrt{T  \log (dT )}\right)
    \end{align}
    for all $T\in \NN_+$.
\end{thm}

The proof of Theorem~\ref{thm:regret} is deferred to Appendix~\ref{app:proof_regret}. Theorem~\ref{thm:regret} establishes that by setting $\alpha$ on the order of $\widetilde{O}\big(\sqrt{T}\big)$, with high probability, the regret of \name is no larger than an order of
$$\widetilde{\gO}\left(d\sqrt{T}\right),$$
assuming the payoff matrix and the noise $\sigma$ are well-bounded.  In particular, when reduced to the linear bandit setting, this matches with the lower bound $\Omega(d\sqrt{T})$ established in  \citet{dani2008stochastic}, suggesting the near-optimality of our result. 
In addition, since $ \min_{t\in[T]}\dualgap{\mu_t,\nu_t}\leq \regret(T) /T$, \name is guaranteed to find an $\varepsilon$-NE of the matrix game \eqref{eq:game_obj} for any $\varepsilon>0$ within $\widetilde{\gO}\left( d^2 /\varepsilon^2 \right)$ samples.

  


